Personalized Jargon Identification for Enhanced Interdisciplinary Communication

Scientific jargon can impede researchers when they read materials from other domains. Current methods of jargon identification mainly use corpus-level familiarity indicators (e.g., Simple Wikipedia represents plain language). However, researchers' familiarity of a term can vary greatly based on their own background. We collect a dataset of over 10K term familiarity annotations from 11 computer science researchers for terms drawn from 100 paper abstracts. Analysis of this data reveals that jargon familiarity and information needs vary widely across annotators, even within the same sub-domain (e.g., NLP). We investigate features representing individual, sub-domain, and domain knowledge to predict individual jargon familiarity. We compare supervised and prompt-based approaches, finding that prompt-based methods including personal publications yields the highest accuracy, though zero-shot prompting provides a strong baseline. This research offers insight into features and methods to integrate personal data into scientific jargon identification.

==> 90-old_formative_study.tex <==
\section{Task Description}
\label{appsec:formative_study}


We conduct an initial study with 10 computer science researchers to (1) validate our intuition that term familiarity is important for interdisciplinary reading, and (2) identify what information needs scholars' have for unfamiliar terms when reading across domains. 

We recruited participants from two subdomains of computer science: Natural-Language Processing (NLP) and Human-Computer Interaction (HCI). Participants were asked to read two pairs of abstracts: an original scientific abstract and a generated abstract personalized to their background. After reading an abstract pair, participants identified what modifications they appreciated in the personalized abstract, and provided a free-text response to whether they preferred the generated abstract and why. 




























\subsection{Initial Findings}

From the 20 responses collected from 10 researchers, 14 expressed a preference for the personalized abstract over the original, with 9 preferring the abstract from the medical domain (90\%) and 5 favoring the related domain (50\%). 

There was a general preference for \textit{adding} information in the personalized abstract over \textit{removing} it (). We categorized participant comments of preferred transformations into four groups:
 

 \begin{itemize}[noitemsep, topsep=1pt, leftmargin=10pt]
    \item \textbf{Background/Motivation} supplies the context, relevance, or rationale for the paper. It may encompass information about the problem being addressed, its significance, the specific research gap it attempts to bridge, or the inspiration behind the research.
    \item \textbf{Definition/Explanation} of crucial terms, concepts, or processes of the research.
    \item \textbf{Method/Result Details} enhance the precision and veracity of the methods and results, e.g., the applied model, data collection processes.
    \item \textbf{Relevant Downstream Connections} provide insights about how the current study can be linked to the reader's own research.
\end{itemize}


While participants had generally positive responses to transformations related to relevant downstream connections (e.g., \ta{TODO}), often these connections were purely hallucinated by the model, which participants were highly critical of ().

Interestingly, many of the other transformations were focused on some term or concept. For example, background and motivation transformations included relevant background on a core concept in the abstract (e.g., \ta{TODO}). Further, participants only wanted additional information if they did not know the term prior to reading the abstract, suggesting that one effective method of personalizing scientific abstracts is through identifying unfamiliar terms and providing relevant informaton (e.g., either additional background or a definition). 

Based on our results, we focus on predicting individual term familiarity and information needs in the context reading scientific abstract's outside of a scholar's domain. 

\lucy{i recommend ending this section on something like: ``Based on these initial findings, we identified the task of individual term familiarity prediction as an important step for scientific abstract personalization. We formalize the task as given an individual scientist defined by their authored publications $P =\{p_1, p_2, ... p_m \}$ and an abstract to personalize $A$, which includes a set of named entities $T =\{t_1, t_2, ... t_n \}$, our goal is to predict the subset of named entities unfamiliar to $P$. In addition, we aim to predict the type of additional information from among \{definition, background, example\} as defined above that $P$ indicated as needed for each unfamiliar entity.'' doesn't have to exactly be this, but i think there needs to be some `output' of the formative study in the form of a task description.}


